Neuro-Symbolic Procedural Planning with Commonsense Prompting

Procedural planning aims to implement complex high-level goals by decomposition into sequential simpler low-level steps. Although procedural planning is a basic skill set for humans in daily life, it remains a challenge for large language models (LLMs) that lack a deep understanding of the cause-effect relations in procedures. Previous methods require manual exemplars to acquire procedural planning knowledge from LLMs in the zero-shot setting. However, such elicited pre-trained knowledge in LLMs induces spurious correlations between goals and steps, which impair the model generalization to unseen tasks. In contrast, this paper proposes a neuro-symbolic procedural PLANner (PLAN) that elicits procedural planning knowledge from the LLMs with commonsense-infused prompting. To mitigate spurious goal-step correlations, we use symbolic program executors on the latent procedural representations to formalize prompts from commonsense knowledge bases as a causal intervention toward the Structural Causal Model. Both automatic and human evaluations on WikiHow and RobotHow show the superiority of PLAN on procedural planning without further training or manual exemplars.

==> input_equation/admissible.tex <==
\begin{equation}
    \reb{{\pi}(s_i|x) = LM_T(LM_G(x))}
    % , \text{where} \ s_i = \{k | k \in [a, o], a \in A, o \in O\}
\end{equation}

==> sections/DONOTUSE-3-method_old.tex <==
\section{Methodology}
\label{sec:method}
\yj{1. problem and SCM high level 2. method }
Our goal is to build a procedural planner to decompose high-level tasks into lower-level time-extended steps. We define a Structural Causal Model of \up{Our \methodname~} in Figure~\ref{fig:SCM} \ww{I'm not sure why you start with SCM here? Also, this forward referencing spans three pages... the readers have to scroll back and forth. I think you should start with figure 1.}, which describes the temporal dynamics and procedural cause-effect relationship. Our causal assumption in SCM indicates that there is a backdoor path from task to steps, which must be blocked with frontdoor adjustment. Therefore, we model the input prompt as a mediator which is created from external commonsense knowledge in a neuro-symbolic approach. This allows us to to prompt the procedural reasoning ability of the language model in a zero-shot setting. The overview of CLAP is shown in Figure~\ref{fig:overview} and the full procedure is shown in Algorithm~\ref{algo:procedure}.

\subsection{Problem Definition}
% We assume a task domain $D_T$, where the agent has certain action set $A$ and the environment contains the object set $O$.
% Each step in the admissible step set $\bar{S}$ is composed of $a \in A$ and $o \in O$.
\reb{Given the high-level task $T$ (e.g. watch television in the living room) sampled from a task domain $D_T$ (e.g. RobotHow), the procedural planning task requires the agent to reason the admissible low-level step $\textbf{S} = \{s_1, ..., s_t | s \in \bar{S}\}$ at each $t$ timestep to complete the task.
% The agent must understand and decompose the high-level task name into admissible low-level steps.
Such task decomposition is achieved by eliciting the knowledge from the large pre-trained language model (LLM) auto-regressively as $P(S_t|D_T, T, A, O, s_{0:t-1})$.
Each $s_t$ is composed of sampled action $a$ and object $o$ from the action set $A$ and the object set $O$ respectively, which satisfy certain affordances in the task domain.\ww{You can add a reference to fig 1 here.}}\xin{we need a new Figure 1 that can serve as a teaser image in the intro. Then you could refer to the new figure without all those distractors in the current figure. }
% which satisfy the affordance property $F$ of each target object $o$.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/overview_v3.pdf}
    \caption{\textbf{\textbf{The} Overview of Procedural Planning.} The architecture is composed of three main components: 1) parsing tasks into structural concept subgraph based on the \reb{external} commonsense knowledge base (Section~\ref{para:step1}). 2) constructing causal mediator with procedural prior (Section~\ref{para:step2}). 3) generating and translating time-extended steps auto-regressively (Section~\ref{sec:method_languageplanning}). D is the unobservable confounding variable in LM_G.
    }
        % \yj{TODO: carefully align each module in the figure with section/paragraph label and highlight to help understanding}
    \label{fig:overview}
\end{figure*}





% \subsection{The Structural Causal Model}
% \label{sec:SCM}
% \noindent \textbf{\reb{Full Temporal Causal Graph}}
% \subsection{\reb{Full Temporal Causal Graph}}




\subsection{\reb{External Knowledge Injection}}
\label{sec:method_concept}
We define our Full Temporal Causal Graph as in Figure~\ref{fig:csm}, which is an unrolled Structural Causal Model (SCM) for sequential decision making. Our goal is to identify the causal effect between \reb{attended task} $T$ and plan procedures $\textbf{S}=\{S_1, S_2,\ldots\}$ from LLMs. 
% In this section, we first introduce the components of our SCM and the logic of our frontdoor adjustment to achieve causal outputs. 
Initially, there are direct paths $T\rightarrow S_i$ and $S_{k}\rightarrow S_i, k<i$ because $S_i$ relies on the \reb{LLM attended task entities} and previous accomplished steps. $D$ is an unobserved confounder from learned knowledge during pre-training. 
% For example, an LLM keeps planning ``find television'' for the task ``read book in the living room'' even if we explicitly indicate the target object in the task name as shown in Figure~\ref{fig:SCM}. 
\reb{$D$ builds a backdoor path between $T$ and $S_i$ and misguides the LLM to attend on false entities to generate the next step (see Fig.~\ref{fig:counterfactual_scm}). Note that $D$ is unobservable as we directly adopt the LLM without knowing the pre-training data}. To mitigate the spurious correlation, we introduce a mediator $P_i$ for each $S_i$ as shown in Figure~\ref{fig:csm} to achieve our frontdoor adjustment
% \noindent \textbf{Causal Intervention} There are two types of operation to control the confounding bias: the \textit{backdoor adjustment} and the \textit{frontdoor adjustment}~\citep{pearl2009causality}. The backdoor adjustment is intractable in our case because it requires the prior distribution of the confounding variables. On the other hand, we can construct an input prompt as a mediator $P_i$ for $T\rightarrow S_i$ and $S_{i-1}\rightarrow S_{i}$. Then the frontdoor adjustment applies a two-step \textit{do}-operation to mitigate bias by investigating $P\rightarrow S_i$~\citep{pearl2009causality}. Specifically, we construct the prompt mediator $P_i$ \reb{using techniques illustrated in Section~\ref{sec:method_concept}}. 
\reb{by injecting \reb{external} commonsense knowledge into LLMs in a neuro-symbolic approach.}

% Though LLMs have strong general language intelligence, they still perform poorly on commonsense reasoning for implementing language planning due to a lack of daily life experience. Inspired by the above causal analysis, we seek to integrate \reb{external} commonsense knowledge into LLMs in a neuro-symbolic approach for causal language planning.
\noindent \reb{\textbf{Step 1: Task-Specific Knowledge Subgraph Sampling}}
\label{para:step1}
In the first step, we investigate the causal effect $T\rightarrow P_i$ and $S_{i-1}\rightarrow P_i$. As a language prompt, $P_i$ inherit the content from $P_{i-1}$ and thus can be detached from steps before $S_{i-1}$ for simplicity. Note that in the path $T\rightarrow D \rightarrow S_i \leftarrow P_i$, $S_i$ is a collider that blocks the association between $D$ and $P_i$. Since there is no backdoor path for $T\rightarrow P_i$ and similarly for $S_{i-1}\rightarrow P_i$, we simply have the conditional probability after applying \textit{do}-operators:
\begin{equation}
\begin{split}
    {P}(P_i=p|do(T)) = {P}(P_i=p|T), \hspace{2ex} {P}(P_i=p|do(S_{i-1})) = {P}(P_i=p|S_{i-1})
    \label{eq:front1}    
\end{split}
\end{equation}
% \noindent \textbf{Step 1}


\reb{To achieve the \textit{do}-operation in a prompting way, we modify the input so that the model can attend on the correct entities. We extract the entities from the task name, and retrieve a one-hop graph from an external knowledge base. The graph can be verbalized and applied as a prompt so that the LLM attends on the correct entities to plan $S_1$.} 
% Note that the prompt is an intermediate reasoning process to induce the output $S_1$ from LLM. 

% For subsequent steps, we append $S_{i-1}$ to $P_i$ so that the LLM is aware of the full step sequences as $P_i$ accumulate over time. For detailed operation, refer to Section~\ref{sec:method_languageplanning}.

\reb{Specifically, in the Semantic Parsing stage (as shown in Figure~\ref{fig:overview}), the high-level task name $T$ is parsed into the entity set $T_E$ with the named entity information to extract the representative nodes from the graph.}
\reb{We use NLTK to tokenize and \texttt{pos\_tag} the task text. Then we use the noun (e.g. television), noun phrases (e.g. remote control) and verb phrases (e.g. watch television) as the entity node.}
% which also exist in the external knowledge graph.
Each entity $e\in T_E$ is used as a query for sampling the local subgraph $G_e \subseteq \mathcal{N}_e \times \mathcal{R}_s \times \mathcal{N}_e$ from the \reb{external} knowledge base $G \subseteq \mathcal{N} \times \mathcal{R} \times \mathcal{N}$ (e.g., ConceptNet~\citep{conceptnet}), where $\mathcal{N}$ and $\mathcal{R}$  represent the number of concept nodes and commonsense relations respectively.
% When extracting subgraphs, the triplets with strong relation (e.g., \texttt{AtLocation}, \texttt{UsedFor}) to the language planning task are kept, while the others are filtered out.
\reb{When extracting subgraphs, we consider the triplets with relation type in household domain (e.g., \texttt{AtLocation}, \texttt{UsedFor}) instead of the linguistic domain (e.g., \texttt{DistinctFrom}, \texttt{DerivedFrom}) to the procedural planning task are kept, while the others are filtered out.}
$\mathcal{N}_e$ is maintained in a set of top-$k$ task-specific nodes using the weight of each $R_e$, which is adapted using the edge-wise invariance module illustrated in the next paragraph.
The global subgraph $G_s$ is a composite of the $\{G_e, e\in E\}$, representing the task-specific \reb{external} knowledge.

\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/SCM1.pdf}
         \caption{Full temporal causal graph}
         \label{fig:csm}
     \end{subfigure}
     \hspace{3ex}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/SCM2.pdf}
         \caption{SCM at step $i$}
         \label{fig:counterfactual_scm}
     \end{subfigure}
        \caption{
        \textbf{Structural Causal Model for Procedural Planning.}
        (a) The full temporal causal graph for procedural planning. $T$ denotes the task query, and $S_i$ denotes the sub-goal step at timestep $i$. $D$ is the unobservable confounding variable introduced by the pre-trained large language model. $P_i$ denotes the mediating variables we construct to mitigate the spurious correlation. (b) The structural causal model at timestep $i$. Without causal intervention, the model produces a sub-goal step ``find television'' due to the spurious correlation between ``television'' and ``living room'' caused by the confounding variable $D$. With our causal intervention, the constructed mediating variable $P_i$ can block the backdoor paths for $T\rightarrow S_i$ and $S_{i-1}\rightarrow S_{i}$ (opened by $D$) and generate the causal sub-goal ``find book'' precisely.
        %\textbf{The Structural Causal Model of Procedural Planning.}(a) the full temporal causal graph for procedural planning. $T$ denotes the task name and $S_i$ denotes the step at timestep $i$. $D$ is the unobservable confounding variable introduced by the pre-training data. $P_i$ denotes the mediating variables we construct to mitigate the spurious correlation. (b) the structural causal model at timestamp $i$. $D$ opens up backdoor paths for $T\rightarrow S_i$ and $S_{i-1}\rightarrow S_{i}$ which can be blocked by introducing $P_i$.
        }
        \label{fig:SCM}
\end{figure}




% \noindent \textbf{Step 2}
\noindent \reb{\textbf{Step 2: Edge-wise Adaption and Symbolic Commonsense Prompt Construction}}
\label{para:step2}
In the second step, we need to find the causal effect for $P_i\rightarrow S_i$. Since the path $P_i\leftarrow T \leftarrow D \rightarrow S_i$ contains a backdoor from $P_i$ to $S_i$, we cannot rely on the conditional probability. Instead, we add intervention on $P_i$ by applying the \textit{do}-operator to cut off $D\rightarrow T$:
\begin{equation}
\begin{split}
    {P}(S_i|do(P_i=p)) &= \sum_{t,s} {P}(S_i|p, T=t, S_{i-1}=s){P}(T=t, S_{i-1}=s)\\
                            &= \sum_{t,s} {P}(S_i|p, T=t, S_{i-1}=s){P}(S_{i-1}=s|T=t)P(T=t)
    \label{eq:front2}
\end{split}
\end{equation}
The retrieved entity-centered graph has multiple edges representing various relationships with other actions/entities. Therefore, the summation over intervened $T$ can be achieved by incorporating these edges into the prompt. For instance, ``living room'' can be ``walked to'' and ``used for reading'' while ``book'' can locate in ``living room'' and ``bedroom''. Similarly, we extrapolate over the edges for $i-1$ hops to aggregate the intervened $S_i$, i.e. $P(S_{i-1}=s|T=t)$.
% We find it effective to implement these interventions in the prompt at the beginning of the planning. 
We refer to this aggregation and conversion to prompt \reb{as \textbf{Edge-wise Adaption} and \textbf{Symbolic Commonsense Prompt Construction}}.
% with more details in Section~\ref{sec:method_concept}.

% \noindent \textbf{Edge-wise Adaption}
% ref: interventional few-shot learning
Directly ranking the retrieved nodes $N_e$ with the pre-computed weight in the \reb{external} knowledge base will result in spurious correlation. Such retrieved local subgraphs tend to capture the task-invariant concept nodes as the causal factors.
To mitigate this, we propose to adapt the weight of each triplet (\reb{\textbf{Edge-wise Adaption}}).
The adaptive weight is the addition of the original edge weight and the cosine similarity between the tail node embedding $\vn_{tail}$ and the task embedding $\vv_{task}$.
\reb{The embeddings are projected from the node text and task name using the sentence-transformer~\citep{reimers-gurevych-2019-sentence} based translation language model $LM_T$.}

% \noindent \textbf{Symbolic Commonsense Prompt Construction}
To better track the utilized \reb{external} knowledge during inference, we construct the task-dependent commonsense prompt with a symbolic program executor (\reb{\textbf{Symbolic Commonsense Prompt Construction}}) guided by the relation type of each triplet in $G_s$ \reb{with the adapted edge weight beyond threshold $\theta_{e}$}.
Specifically, the executor acquires the neural information of each natural language node and executes the sequential mapping program \reb{by sampling the operation $Op$ from the Symbolic Rule Set $R$} according to the edge relation type.
% Symbolic Rule Set $R$
\reb{For instance, the $AtLocation$ edge samples the operation \texttt{Op\_AtLocation} from $R$, which} takes the commonsense relation of the triplet from $G_s$ as the parameters to query the procedural concept output given the natural language meaning of the linked nodes (e.g., go to the location of \texttt{Start\_Node\_Of}($r_e$) in this case).
Similarly, \texttt{Op\_UsedFor} may refer to "go to find \texttt{End\_Node\_Of}($r_e$) and use it for \texttt{Start\_Node\_Of}($r_e$)".
And operators \texttt{Op\_HasSubevent} and \texttt{Op\_HasPrerequisite} will recursively navigate the subgraph $G_e$.
\reb{After navigating the subgraph, we linearize the transformed triplets as the final \textbf{Symbolic Commonsense Prompt $P_G$}, which is then translated to \textbf{Admissible Knowledge $\hat{P_G}$} by the translation language model $LM_T$.}

% =============
Combining the two steps, we can obtain a prompt with aggregation of \reb{external} knowledge in a procedural script format. The underlying causal mechanism is a combination of Eq.~\ref{eq:front1} and Eq.~\ref{eq:front2}:
\begin{equation}
\begin{split}
    {P}(S_i|do(T),\reb{do(S_{i-1})} ) &= \sum_{p} {P}(S_i|do(P_i=p)){P}(p|do(T), do(S_i))\\
    &=\sum_{p} {P}(p|T) \sum_{t,s} {P}(S_i|p, T=t, S_{i-1}=s){P}(T=t, S_{i-1}=s)
    \label{eq:frontdoor}
\end{split}    
\end{equation}
\reb{The adjustment and marginalization in Eq.~\ref{eq:frontdoor} is achieved in the input space by forming neuro-symbolic prompts that allows the LLM to attend on the causal entities instead of the highly correlated ones for next step prediction. We relates the task entities with abundant concepts from an external knowledge base originally in a graph format. The LLM can reason over the most relevant edges to link the concepts with the task entities as a context.} \reb{The prompts from knowledge bases are independent of the pre-training data distribution so that $P_i$ is independent of $D$ and satisfies the frontdoor criterion. Please refer to Appendix~\ref{sec:theoretical_details} for more details on the simplification of our causal temporal graph.}



\begin{algorithm}[t]
\caption{Neuro-Symbolic Procedural Planning using Commonsense-Infused Prompting
}
\label{algo:procedure}
\begin{algorithmic}[1]

\REQUIRE ~~\\ %Input
Task Dataset $\mathcal{D}$, Admissible Step Set $S$, \reb{External} knowledge Graph $G$;\\
Language Model for Generation $LM_G$ and Translation $LM_T$, Symbolic Rule Set $R$; \\
\ENSURE ~~\\ %Output
\STATE Zero-shot Inference for Temporal-extended Procedure Plan $S_T = {s_1, ..., s_t}$;
\FOR{each Task Sample $T$ in $\mathcal{D}$}
\STATE Semantically parse $T$ into entity set $T_E$;
\STATE Retrieve commonsense subgraph $G_s$ from $G$ for each $e \in T_E$;
\STATE Construct procedural commonsense knowledge $P_G$ based on $G_s$ using Symbolic Rule Set $R$;
\STATE Translate $P_G$ in Admissible Knowledge $\hat{P_G}$ = $LM_T (P_G)$;
\STATE Prompt $P$ $\leftarrow$ Initial task name $T$ + \reb{External} Knowledge $\hat{P_G}$;
\FOR{each timestep $t$}
\STATE $s_t$ = $LM_T (LM_G (P_t))$;
\STATE Update Procedure Plan $S_T$ $\leftarrow$ $s_t$, Update Prompt $P_{t+1}$ $\leftarrow$ $s_t$;
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[b]{0.35\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SCM1.pdf}
%          \caption{Full temporal causal graph}
%          \label{fig:csm}
%      \end{subfigure}
%      \hspace{3ex}
%      \begin{subfigure}[b]{0.6\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SCM2.pdf}
%          \caption{SCM at step $i$}
%          \label{fig:counterfactual_scm}
%      \end{subfigure}
%         \caption{\textbf{The Structural Causal Model of our Language Planner.}
%         (a) the full temporal causal graph for language planning. $T$ denotes the task name and $S_i$ denotes the step at timestep $i$. $D$ is the unobservable confounding variable introduced by the pre-training data. $P_i$ denotes the mediating variables we construct to mitigate the spurious correlation. (b) the structural causal model at timestamp $i$. $D$ opens up backdoor paths for $T\rightarrow S_i$ and $S_{i-1}\rightarrow S_{i}$ which can be blocked by introducing $P_i$.
%         }
%         \label{fig:SCM}
% \end{figure}


\subsection{Procedural Planning}
\label{sec:method_languageplanning}
\noindent \textbf{Semantic Generation}
The \reb{external} knowledge is further concatenated with the high-level task name as the initial prompt.
\reb{The initial prompt contains limited semantics and executability, but still contains external knowledge and structure that help leverage the reasoning ability of the large language models.}
Given the prompt, the language model \reb{$LM_G \in \{P_{AR}, P_{AE}\}$} generates the next sentence, and the most confident prediction is then appended to previous prompts.
The language model terminates when reaching the max step $t$ or has confidence below threshold $\theta$. The joint probabilities of \reb{auto-regressive ($P_{AR}$) and auto-encoder ($P_{AE}$) model} is factorized as:
\begin{equation}
    P_{AR}(x) = \prod_{i=1}^{n}p(s_n|\reb{\hat{P_G}}, s_{1:n-1}, \reb{T}) , \hspace{2ex} P_{AE}(x) = \prod_{i=1}^{n}p(s_n|\reb{\hat{P_G}}, \{s_{1:n-1}, [MASK]\}, \reb{T})
\end{equation}
\reb{where $\hat{P_G}$ represent the commonsense knowledge and $T$ represent the task name.}

\noindent \textbf{Admissible Step Translation}
Procedural planning requires grounding the step into an admissible composite of action and object.
\reb{To ensure that the generated language plans could ground to the specific task domain (e.g. RobotHow, WikiHow), we should avoid to produce the steps that are inadmissible (e.g. Toast the table).
In other words, the generated steps should be fully constrained to admissible ones.
Thus previous works (~\citep{wenlong2022planner, ahn2022can}) have explored to use the model (which is ${LM_T}$ in our case) to score a step selected from a fixed set of available options, instead of directly sampling from the output distributions of the language model (which is ${LM_G}$ in our case).
Specifically, the Admissible Step Translation is conducted by mapping the generated step by ${LM_G}$ into admissible step by matching based on the similarity in the Sentence-Transformer ~\citep{reimers-gurevych-2019-sentence} (${LM_T}$) embedding space.}
% following the baseline \planner~(~\citep{wenlong2022planner})
Following~\citep{wenlong2022planner}, \reb{we utilize a sentence-transformer based translation language model $LM_T$ for semantic matching with cosine similarity:}
\begin{equation}
    P(s_i|x) = LM_T(LM_G(x)), \text{where} \ s_i = \{k | k \in [\reb{a}, o], \reb{a \in A}, o \in O\}
\end{equation}
\reb{which translates $LM_G(x)$ into the admissible step $s_i \in S$ that is the closest in the embedding space measured by the cosine similarity.}
\reb{$A$ and $O$ represent the action set and object set respectively.}
% The language model $LM_G \in \{P_{AR}, P_{AE}\}$ is either the autoencoder or autoregressive architecture.

\subsection{Counterfactual Procedural Data Construction}
To investigate the counterfactual reasoning ability of the procedural planning models, we design \up{three} families of intervention methods: 1) \textbf{Initial Configuration}: intervene the initial configuration, such as the location for implementing the task. 2) \textbf{Intermediate Step}, randomly selecting the step from the program as an additional constraint \reb{the task name} for implementing the task. 3) \textbf{Final Goal}, intervene the task goal as the composite of another randomly sampled task.
The counterfactual dataset construction details and \reb{post-intervention examples are provided in Appendix~\ref{sec:counterfactual_construction}.}


==> sections/DONOTUSE-3-methodbefore.tex <==
\section{Methodology}
\label{sec:method}
Our goal is to build a language planner to decompose high-level tasks into lower-level time-extended steps. We define a Structural Causal Model of \up{Our \methodname~} in Figure~\ref{fig:SCM}, which describes the temporal dynamics and procedural cause-effect relationship. Our causal assumption in SCM indicates that there is a backdoor path from task to steps, which must be blocked with frontdoor adjustment. Therefore, we model the input prompt as a mediator which is created from external commonsense knowledge in a neuro-symbolic approach. This allows us to to prompt the procedural reasoning ability of the language model in a zero-shot setting. The overview of CLAP is shown in Figure~\ref{fig:overview} and the full procedure is shown in Algorithm~\ref{algo:procedure}.

\subsection{Problem Definition}
We assume a task domain $D_T$, where the agent has certain action set $A$ and the environment contains the object set $O$.
Each step in the admissible step set $\bar{S}$ is composed of $a \in A$ and $o \in O$.
Given the high-level task $T$ sampled from $D_T$, the agent needs to reason the steps $\textbf{S} = \{s_1, ..., s_t | s \in \bar{S}\}$ for $t$ timesteps to achieve the final goal. 
The agent must understand and decompose the high-level task name into admissible low-level steps. 
This transition is achieved by eliciting the knowledge from the large pre-trained language model (LLM) auto-regressively as $P(S_t|D_T, T, A, O, s_{0:t-1})$. The reasoned $s$ should satisfy certain constraints, including the action set, and the object set, which satisfy the affordance property $F$ of each target object $o$.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/overview_v2.pdf}
    \caption{\textbf{\textbf{The} Overview of Causal Language Planner.} The architecture is composed of three main components: 1) parsing tasks into structural concept subgraph based on the \reb{external} commonsense knowledge base. 2) constructing causal mediator with procedural prior. 3) generating and translating time-extended steps auto-regressively. 
    }
    \label{fig:overview}
\end{figure*}

\begin{algorithm}[t]
\caption{Neuro-Symbolic Causal Procedural Planning using Commonsense-Infused Prompting
}
\label{algo:procedure}
\begin{algorithmic}[1]

\REQUIRE ~~\\ %Input
Task Dataset $\mathcal{D}$, Admissible Step Set $S$, \reb{External} knowledge Graph $G$;\\
Language Model for Generation $LM_G$ and Translation $LM_T$, Symbolic Rule Set $R$; \\
\ENSURE ~~\\ %Output
\STATE Zero-shot Inference for Procedure $S_T = {s_1, ..., s_t}$;
\FOR{each Task Sample $T$ in $\mathcal{D}$}
\STATE Parse $T$ into entity set $T_E$;
\STATE Retrieve commonsense subgraph $G_s$ for each $e \in T_E$;
\STATE Construct procedural commonsense knowledge $P_G$ using Symbolic Rule Set $R$;
\STATE Translate $P_G$ in Admissible Knowledge $\hat{P_G}$ = $LM_T (P_G)$;
\STATE Prompt $P$ $\leftarrow$ Initial task name $T$ + \reb{External} Knowledge $\hat{P_G}$;
\FOR{each timestep $t$}
\STATE $s_t$ = $LM_T (LM_G (P_t))$;
\STATE Generated procedure $S_T$ $\leftarrow$ $s_t$, Prompt $P_{t+1}$ $\leftarrow$ $s_t$;
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{The Structural Causal Model}
\label{sec:SCM}
We define our Full Temporal Causal Graph as in Figure~\ref{fig:csm}, which is an unrolled Structural Causal Model (SCM) for sequential decision making. Our goal is to identify the causal effect between task $T$ and plan procedures $\textbf{S}=\{S_1, S_2,\ldots\}$ from LLMs. In this section, we first introduce the components of our SCM and the logic of our frontdoor adjustment to achieve causal outputs. 

\noindent \textbf{Full Temporal Causal Graph} Procedural planning is to generate a sequence of procedures where the causal effect is denoted as $T\rightarrow \textbf{S}$. Initially, there are direct paths $T\rightarrow S_i$ and $S_{k}\rightarrow S_i, k<i$ because $S_i$ relies on the task name and previous accomplished steps. $D$ is a confounder from pre-trained knowledge. For example, an LLM keeps planning ``find television'' for the task ``read book in the living room'' even if we explicitly indicate the target object in the task name as shown in Figure~\ref{fig:SCM}. We conjecture that the pre-trained knowledge builds a spurious correlation between ``living room'' and ``TV'', which is unobservable in the latent space of the LLM. Therefore, to mitigate this issue, we introduce a mediator $P_i$ for each $S_i$ as shown in Figure~\ref{fig:csm} to achieve our frontdoor adjustment. 

\noindent \textbf{Causal Intervention} There are two types of operation to control the confounding bias: the \textit{backdoor adjustment} and the \textit{frontdoor adjustment}~\citep{pearl2009causality}. The backdoor adjustment is intractable in our case because it requires the prior distribution of the confounding variables. On the other hand, we can construct an input prompt as a mediator $P_i$ for $T\rightarrow S_i$ and $S_{i-1}\rightarrow S_{i}$. Then the frontdoor adjustment applies a two-step \textit{do}-operation to mitigate bias by investigating $P\rightarrow S_i$~\citep{pearl2009causality}. Specifically, we construct the prompt mediator $P_i$ \reb{using techniques illustrated in Section~\ref{sec:method_concept}}. 

In the first step, we investigate the causal effect $T\rightarrow P_i$ and $S_{i-1}\rightarrow P_i$ as shown in Figure~\ref{fig:SCM}. As a language prompt, $P_i$ inherit the content from $P_{i-1}$ and thus can be detached from steps before $S_{i-1}$ for simplicity. Note that in the path $T\rightarrow D \rightarrow S_i \leftarrow P_i$, $S_i$ is a collider that blocks the association between $D$ and $P_i$. Since there is no backdoor path for $T\rightarrow P_i$ and similarly for $S_{i-1}\rightarrow P_i$, we simply have the conditional probability after applying \textit{do}-operators:
\begin{equation}
\begin{split}
    {P}(P_i=p|do(T)) = {P}(P_i=p|T), \hspace{2ex} {P}(P_i=p|do(S_{i-1})) = {P}(P_i=p|S_{i-1})
    \label{eq:front1}    
\end{split}
\end{equation}
\noindent \textbf{Step 1} To make the LLM attend to the right cause and avoid spurious correlation, we extract the entity, e.g. ``book'' from the task name, and retrieve a graph from an external knowledge base. This graph, centralized at ``book'', can be verbalized and used as a prompt so that the LLM concentrates on the right location to plan $S_1$. Note that the prompt is an intermediate reasoning process to induce the output $S_1$ from LLM. For subsequent steps, we append $S_{i-1}$ to $P_i$ so that the LLM is aware of the full step sequences as $P_i$ accumulate over time. For detailed operation, refer to Section~\ref{sec:method_languageplanning}.

\noindent \textbf{Step 2} In the second step, we need to find the causal effect for $P_i\rightarrow S_i$. Since the path $P_i\leftarrow T \leftarrow D \rightarrow S_i$ contains a backdoor from $P_i$ to $S_i$, we cannot rely on the conditional probability. Instead, we add intervention on $P_i$ by applying the \textit{do}-operator to cut off $D\rightarrow T$:
\begin{equation}
\begin{split}
    {P}(S_i|do(P_i=p)) &= \sum_{t,s} {P}(S_i|p, T=t, S_{i-1}=s){P}(T=t, S_{i-1}=s)\\
                            &= \sum_{t,s} {P}(S_i|p, T=t, S_{i-1}=s){P}(S_{i-1}=s|T=t)P(T=t)
    \label{eq:front2}
\end{split}
\end{equation}
The retrieved entity-centered graph has multiple edges representing various relationships with other actions/entities. Therefore, the summation over intervened $T$ can be achieved by incorporating these edges into the prompt. For instance, ``living room'' can be ``walked to'' and ``used for reading'' while ``book'' can locate in ``living room'' and ``bedroom''. Similarly, we extrapolate over the edges for certain hops to aggregate the intervened $S_i$, i.e. $P(S_{i-1}=s|T=t)$. We find it effective to implement these interventions in the prompt at the beginning of the planning. 
We refer to this aggregation and conversion to prompt \reb{as two components, \textbf{Edge-wise Adaption} and \textbf{Symbolic Commonsense Prompt Construction}} with more details in Section~\ref{sec:method_concept}.
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/SCM1.pdf}
         \caption{Full temporal causal graph}
         \label{fig:csm}
     \end{subfigure}
     \hspace{3ex}
     \begin{subfigure}[b]{0.6\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/SCM2.pdf}
         \caption{SCM at step $i$}
         \label{fig:counterfactual_scm}
     \end{subfigure}
        \caption{\textbf{The Structural Causal Model of our Language Planner.}
        (a) the full temporal causal graph for procedural planning. $T$ denotes the task name and $S_i$ denotes the step at timestep $i$. $D$ is the unobservable confounding variable introduced by the pre-training data. $P_i$ denotes the mediating variables we construct to mitigate the spurious correlation. (b) the structural causal model at timestamp $i$. $D$ opens up backdoor paths for $T\rightarrow S_i$ and $S_{i-1}\rightarrow S_{i}$ which can be blocked by introducing $P_i$.
        }
        \label{fig:SCM}
\end{figure}

Combining the two steps, we can obtain a prompt with aggregation of \reb{external} knowledge in a procedural script format. The underlying causal mechanism is a combination of Eq.~\ref{eq:front1} and Eq.~\ref{eq:front2}:
\begin{equation}
\begin{split}
    {P}(S_i|do(T)) &= \sum_{p} {P}(S_i|do(P_i=p)){P}(p|do(T), do(S_i))\\
    &=\sum_{p} {P}(p|T) \sum_{t,s} {P}(S_i|p, T=t, S_{i-1}=s){P}(T=t, S_{i-1}=s)
    \label{eq:frontdoor}
\end{split}    
\end{equation}
The effect of introducing the dedicated prompt can be interpreted as an intermediate process where the LLM relates the task entities with all concepts from an external knowledge base in a graph format. Then it reasons over the most relevant edges to link the entities with the task name as a context. The prompts from knowledge bases are independent of the pre-training knowledge so that $P_i$ satisfies the frontdoor criterion. Please refer to Appendix~\ref{sec:theoretical_details}. The following sections explain how the causal model and frontdoor adjustment are implemented in detail. 


\subsection{\reb{External} Knowledge Injection}
\label{sec:method_concept}
Though LLMs have strong general language intelligence, they still perform poorly on commonsense reasoning for implementing procedural planning due to a lack of daily life experience. Inspired by the above causal analysis, we seek to integrate \reb{external} commonsense knowledge into LLMs in a neuro-symbolic approach for causal procedural planning.

\noindent \textbf{Task-Specific Subgraph Sampling} To extract the representative nodes from the graph, the high-level task name $T$ is parsed into the entity set $T_E$ with the help of the named entity information.
\reb{We use nltk to tokenize and pos\_tag the task string and filter the noun as the atomic entity node. In addition we extract noun phrases and verb phrases as compositional node, which also exist in the external knowledge graph.}
Each entity $e\in T_E$ is used as a query for sampling the local subgraph $G_e \subseteq \mathcal{N}_e \times \mathcal{R}_s \times \mathcal{N}_e$ from the \reb{external} knowledge base $G \subseteq \mathcal{N} \times \mathcal{R} \times \mathcal{N}$ (e.g., ConceptNet~\citep{conceptnet}), where $\mathcal{N}$ and $\mathcal{R}$  represent the number of concept nodes and commonsense relations respectively.
% When extracting subgraphs, the triplets with strong relation (e.g., \texttt{AtLocation}, \texttt{UsedFor}) to the language planning task are kept, while the others are filtered out.
\reb{When extracting subgraphs, we consider the triplets with relation type in household domain (e.g., \texttt{AtLocation}, \texttt{UsedFor}) instead of the linguistic domain (e.g., \texttt{DistinctFrom}, \texttt{DerivedFrom}) to the procedural planning task are kept, while the others are filtered out.}
$\mathcal{N}_e$ is maintained in a set of top-$k$ task-specific nodes using the weight of each $R_e$, which is adapted using the edge-wise invariance module illustrated in the next paragraph.
The global subgraph $G_s$ is a composite of the $\{G_e, e\in E\}$, representing the task-specific \reb{external} knowledge.

\noindent \textbf{Edge-wise Adaption}
% ref: interventional few-shot learning
Directly ranking the retrieved nodes $N_e$ with the pre-computed weight in the \reb{external} knowledge base will result in spurious correlation. Such retrieved local subgraphs tend to capture the task-invariant concept nodes as the causal factors.
To mitigate this, we propose to adapt the weight of each triplet.
The adaptive weight is the addition of the original edge weight and the cosine similarity between the tail node embedding $\vn_{tail}$ and the task embedding $\vv_{task}$. \reb{The embeddings are projected from the node text and task name using the sentence-transformer~\citep{reimers-gurevych-2019-sentence} based translation language model $LM_T$.}

\noindent \textbf{Symbolic Commonsense Prompt Construction} To better track the utilized \reb{external} knowledge during inference, we construct the task-dependent commonsense prompt with a symbolic program executor guided by the relation type of each triplet in $G_s$ \reb{with the adapted edge weight beyond threshold $\theta_{e}$}.
Specifically, the executor acquires the neural information of each natural language node and executes the sequential mapping program \reb{by sampling the operation $Op$ from the Symbolic Rule Set $R$} according to the edge relation type.
% Symbolic Rule Set $R$
\reb{For example, the edge with $AtLocation$ type samples the operation \texttt{Op\_AtLocation} from $R$, which} takes the commonsense relation of the triplet from $G_s$ as the parameters to query the procedural concept output given the natural language meaning of the linked nodes (e.g., go to the location of \texttt{Start\_Node\_Of}($r_e$) in this case).
Similarly, \texttt{Op\_UsedFor} may refer to "go to find \texttt{End\_Node\_Of}($r_e$) and use it for \texttt{Start\_Node\_Of}($r_e$)".
And operators \texttt{Op\_HasSubevent} and \texttt{Op\_HasPrerequisite} will recursively navigate the subgraph $G_e$.
\reb{After navigating the subgraph, we linearize the transformed triplets as the final \textbf{Symbolic Commonsense Prompt $P_G$}, which is then translated to \textbf{Admissible Knowledge $\hat{P_G}$} by the translation language model $LM_T$.}

\subsection{Procedural Planning}
\label{sec:method_languageplanning}
\noindent \textbf{Semantic Generation}
The \reb{external} knowledge is further concatenated with the high-level task name as the initial prompt.
\reb{The initial prompt contains limited semantics and executability, but still contains external knowledge and structure that help leverage the reasoning ability of the large language models.}
Given the prompt, the language model \reb{$LM_G \in \{P_{AR}, P_{AE}\}$} generates the next sentence, and the most confident prediction is then appended to previous prompts.
The language model terminates when reaching the max step $t$ or has confidence below threshold $\theta$. The joint probabilities of \reb{auto-regressive ($P_{AR}$) and auto-encoder ($P_{AE}$) model} is factorized as:
\begin{equation}
    P_{AR}(x) = \prod_{i=1}^{n}p(s_n|c, s_{1:n-1}, t) , \hspace{2ex} P_{AE}(x) = \prod_{i=1}^{n}p(s_n|c, \{s_{1:n-1}, [MASK]\}, t)
\end{equation}
\noindent \textbf{Admissible Step Translation}
Procedural planning requires grounding into an admissible composite of actions and target objects.
Following~\citep{wenlong2022planner}, we utilize a sentence-transformer based translation language model $LM_T$ via a semantic matching as:
\begin{equation}
    P(s_i|x) = LM_T(LM_G(x)), \text{where} \ s_i = \{k | k \in [v, o], v \in V, o \in O\}
\end{equation}
which translates the generated language embedding into the admissible step $s_i \in S$.
% The language model $LM_G \in \{P_{AR}, P_{AE}\}$ is either the autoencoder or autoregressive architecture.

\subsection{Counterfactual Procedural Data Construction}
To investigate the counterfactual reasoning ability of the procedural planning models, we design \up{three} families of intervention methods: 1) \textbf{Initial Configuration}: intervene the initial configuration, such as the location for implementing the task. 2) \textbf{Intermediate Step}, randomly selecting the step from the program as an additional constraint for implementing the task. 3) \textbf{Final Goal}, intervene the task goal as the composite of another randomly sampled task.
The counterfactual dataset construction details and examples are provided in Appendix~\ref{sec:counterfactual_construction}.


==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section xxx.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{sec:intro}}
  \item Did you describe the limitations of your work?
    \answerYes{See Appendix~\ref{sec:limitations} in supplemental materials.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Appendix~\ref{sec:ethical} in supplemental materials.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec:method_concept} and Appendix~\ref{sec:theoretical_details}}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix~\ref{sec:theoretical_details}}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We are cleaning up our codebase, and we plan to release the code/data/instructions in the camera-ready version of our paper.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:exp_setup} and Appendix~\ref{sec:implementation_details}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec:computation}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{sec:exp_setup} dataset.}
  \item Did you mention the license of the assets?
    \answerYes{See Section~\ref{sec:exp_setup} dataset.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See Appendix~\ref{sec:counterfactual_construction} for new asset examples, we are cleaning up the data pipeline, and we plan to release the full new assets in the camera-ready version of our paper.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{The dataset is publicaly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{The dataset is household content without personal information.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See Appendix~\ref{sec:amazon_mechanical_turk}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{No potential risks in this work to our best knowledge. And no human subject study involved in this work.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See Appendix~\ref{sec:amazon_mechanical_turk}}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/rebuttal.tex <==
# Rebuttal

## Response to Official Review of Paper822 by Reviewer W99u
### Weaknesses
> **R1W(eakness)1.** It's not clear which is the current causal model used at each point. (See question below)

As for the timestep-wise causal model (e.g., SCM when predicting Step 1 at each **iteration**), Figure 2(b) show the general SCM at step $i$, and Figure 4(a)(b)(c) show more detail of the difference between the SCM at initial timestep (timestep $i$=1) and the following timesteps (timestep $i$>1). We also add the reference to the SCM for each stage in Algorithm 1 in the revision.
As for the operation-wise causal model (e.g., SCM before and after each **equation** at each iteration), we add a new Figure 4 in Appendix A.3 to show how the SCM transit before and after each equation.

> **R1W2.**   The paper might be assuming $P_i$ is the only path, but the existence of other paths to be blocked it's not discussed.

As one assumption of the front-door criterion is that the only way in which the task name $T$ influences $S_i$ is through the mediator $P_i$. Thus $P_i$ must be the only path, otherwise the front-door adjustment cannot stand.

> **R1W3.** The argument loses a bit in the adaptation plus other decisions on what to retrieve.

The Edge-Wise Adaption is an implementation of the $do$-operator on $P_i$ by adjusting the weight of the edge in the external knowledge graph. The external knowledge graph $G$ already annotate the weight of each edge ($E_w$). The edge link entity nodes in the graph. We argue that the annotated weight will result in a spurious correlation, since they capture the task-invariant concept nodes as the causal factors.
Thus we addtionally consider the semantic relatedness between the node embedding in the graph with the task embedding. Specifically, we adapt the original $E_w$ by the addition of $E_w$ and the cosine similarity of node embedding and task embedding as: $\hat{E_w} \leftarrow E_w + cosine(n_{E_{tail}}, v_{task})$, where $n_{E_{tail}}$ is the tail node embedding of the edge $R_e$ and $v_{task}$ the task embedding. We re-write the paragraph about Edge-wise Adaption with above details in Stage 2 paragraph in Section 3.1.
The nodes $N_e$ are retrieved by ranking the adaptative weight $\hat{E_w}$. Since the nodes linked with these highly-weighted edge are most likely to provide commonsense knowledge for generating the procedural plan for the task. We decide to retrieve $3$-hop subgraph for two reasons: 1) there is a limit of input sequence length for the LLMs 2) the downgraded relatedness of the node that is multi-hops away from the entity nodes parsed from the task $T$, as previous work using ConceptNet also observe the same trend and also decide to do $3$-hop subgraph retrieval ([1]).
We add more details of the adaption and decisions on what to retrieve in Stage 2 paragraph in Section 3.1 and Appendix B.2. 

[1] Xikun Zhang, AntoineXikun Zhang, Antoine Bosselut, Michihiro Yasunaga, Hongyu Ren, Percy Liang, Christopher D. Manning, Jure Leskovec, "GreaseLM: Graph REASoning Enhanced Language Models for Question Answering", ICLR 2022

### Clarity, Quality, Novelty And Reproducibility
#### Clarity of Causal Analysis
> **R1C(larity)1.** Clarity of the Equations (Eq.1, Eq.10 (now Eq. 9 in revision) and Eq.9 (now Eq. 8 in revision)) in paper compared with using the causalfusion tool.

We thank reviewer to bring out the comparison between the estimands from the tool and our equations. And yes, the model in Figure 2 is updated after each iteration with fixed values of previous variables. For example, at timestep $i$, the $T$ and $P_{i-1}$ are fixed and do not require further prediction. In other words, we're actually doing timestep-wise greedy decoding (each step $S_i$ is greedy decoded at each timestep $i$). Notice that at token-wise, we keep the decoding unchanged for LLM.

> **R1C2.** Refer to the causal models in the equations.

We add the details of both timestep-wise causal model (what's the SCM at each timestep) and operation-wise causal model (what's the SCM before and after each equation) in Figure 4 in Appendix A.3. Please also refer to the response at **R1W(eakness)1.**

#### Clarity of the algorithm as well as the prediction of all the do() compounded
> **R1C3.** What's exactly the new causal graph after each iteration.

Please refer to "timestep-wise causal model " in the response at **R1W(eakness)1.**, where we explain more on how Figure 2, Figure 4 a show the causal graph after each iteration (timestep-wise). Basically, the causal graph at timestep $i = 1$ is shown in Figure 4(a) and the causal graph at timestep $i > 1$ is shown in Figure 4(b). During each iteration, the system go through several operations, and the operation-wise change on causal graph is shown in a new added Figure 5.

> **R1C4.** Why does it make sense to simplify the graph.

We simplyfy the causal graph at timestep $i$ ($i$ > 1) in Figure 4(b) into Figure 4(c) in Appendix A.3. After simplification based on Equation 12-16, we get the SCM at timestep $i>1$ in Figure 4(b). This is an equivalent SCM after eliminating $P_{i-1}$ in Figure 4(c).
The reason we could eliminate $P_{i-1}$ is as follows. We follow a common method of constructing temporally-extended prompt, which is to append the prediction at previous timesteps to the prompt at current timestep. In our case, the $P_{G, i}$ is the same as $P_{G, i-1}$, thus $P_i$ inherit part of the content from $P_{i-1}$, the change only depend on the $S_{i-1}$. Thus $P_{i-1}$ and $S_{i-2}$ are fixed, and there is no need to predict $P_{i-1}$ at timestep $i$ again. In this way, we simplyfiy the causal graph in Figure 4(b) to the one in Figure 4(c). In summary, we define and simplify the causal graph based on the temporall-extended property of our prompt construction ($P_{i}$ inherit the content from $P_{i-1}$).
We extend above clarity of definition paragraph in Appendix A.3.

> **R1C5.** Clarify which causal graph is related to each equation.

Please refer to "operation-wise causal model" in the response to the response at **R1W(eakness)1.**. We clarify this with a new added Figure 5 in Appendix A.3 about the SCM after each equation (operation-wise).

#### More Questions
> **R1Q(uestion)1.** does the causal analysis holds given de "adaption" that was necessary? I'd like to see a more clear causal criticism of that situation.

The Edge-wise Adaption is actuall an implementation of the $do$-operator on $P_i$ by adjusting the weight of the edge in the external knowledge graph. Please refer the revision paper and also response to the third weakness for the expanded details of the adpation module. The causal analysis still holds given that the adpation is to intervene $P_i$ as a part of front-door adjustment instead of changing the situation.

> **R1Q2.** Does the use of the front criterion holds given that there could exist other words related to the task?

If I'm understanding your question correctly, you're asking the situation that different words can describe the same task.
For example, one possible situation is that the words "watch the TV" is the synonym of the words "watch the television".  In this case, with the help of synonym relation reconginized in the external resource (e.g., ConceptNet), we could retrieve the same subgraph.
Another possible situation is that the words related to the tasks are semantically relevant but not recognized as the synonymys in the external resources. In this case, since we're still fixing the task $T$ and ground truth procedural plan, the constructed prompt $P_i$ as the mediator intercepts all directed paths from $T$ to $S_i$. Thus the front-door criterion still hold in above both situations.

> **R1Q3.**  Where would this break? The results are just positive but there is not a detailed discussion on limitations.

We discuss about the limitations in Appendix E.1, where we mainly talked about the difficulty of reasoning long-horizon, complex, or composite procedural plan. We also talked about inherent differences among multiple langauges may result in differed planning strategies in granularity or abstraction levels.

Above limitations are discussed mainly based on the challenges of procedural planning task. In addition, there are limitations of our implementation that is guided by our causal analysis. First, the coverage of the leveraged external resources is limited, which is common in knowledge-enhanced system. This may result in the wrong understanding of the task and produce not reasonable procedural plans. For example, the knowledge of the word "Turking", which refers to "The act or process of performing small tasks using the Amazon Mechanical Turk service." according to Wiktionary, is not covered in the external resources (e.g., ConceptNet). Since our proposed system do not assume specific external resources. It's doable in the future that we utilize more powerful external resources (e.g., Wiktionary). Second, the hop number and the threshold of the multi-hop retrieval in task-relevant subgraph sampling is currently a configured hyperparameter. This may result in not ideally constructed prompt. The future work could instead make these hyperparameters learnable on each task domain, and also explore the pros and cons between end-to-end commonsense-infused prompt versus neuro-symbolic constructed prompt.
We extend Appendix E.1 with above discussions in the revision.

## Response to Official Review of Paper822 by Reviewer UWNS
### Weaknesses

> **R2W(eakness)1.** The clarity could be improved. Some sections like Section 3 are quite dense and difficult to parse, particularly Section 3.1. Perhaps an earlier overview could help clarify or explicit running examples. Section 3.1 could use it’s own algorithm block and potentially a zoomed in figure of the computation. Figure 3, though a nice overview, is very dense.

We extend the paragraph at the begging of Section 3 and add an earlier overview paragraph of Section 3.1 with more clarity and explicit running examples in Appedix D.2 to help parse Section 3.
We expand Algorithm 1 with a fine-grained algorithm block for Secion 3.1 that show the computation flow.

>  **R2W2.** Though the performance of PLAN is stronger than baselines, it is a smaller improvement than I would think given the additional complexity and also somewhat difficult to judge how large of an improvement it is. In many of the metrics it seems PLAN outperforms by a few percentage points or in voting it wins 50% of the time. While I acknowledge that this shows that PLAN is performing better, it isn’t clear from these results that it is worth the vast additional complexity compared to baselines. The authors should add an additional metric similar to executability in Huang et al., showing the actual success rate of these plans, as this is the ultimate metric we care about.

We thank the reviewer for point out the concerns about the complexity and ultimate evaluation metric above. We'll address them point by point:
 1. Concern about brought in complexity for the improvement. Whether it's worth the vast additional complexity compared to the baselines.

As can be seen in both automatic and human evaluation, our method consistently surpass the baselines and achieve a very good performance especially in win-tie-lose experiment. As for the complexity, after the thorough causal analysis, we come to a implementation that automatically leverage the external knowledge instead of require additional exemplars.
And we provide the quantitative analysis of time cost comparison in Table 8 and Table 9 (the last column) in Appendix C.2, indicating the comparable computational complexity of our method and baselines. Thus we claim that the brought in complexity is ignorable and is worth for the improvement we achieve.

 2. Difficult to judge the improvement. An additional metric to show the actual success rate of the plans.

As for the automatic evaluation metric, the most human-correlated one is the BERT-score. But our most important metrics are still human evaluation, especially the Win-Tie-Lose experiment.
In Table 12, we add a new human metric to show whether the procedural plans can successfully implement the task. The consistent improvement over human metrics that evaluate coverage, order and success rate is more convincing to prove the contribution of our work.
The details of new evaluation results with new added success rate metric is discussed in a new added paragraph "Evaluation on Success Rate Metric" in Appendix C.2.


> A few related questions:
> **R2W(eakness)2R(elated)Q(uestion)1.** I would be interested to learn more about what the main failure modes are.

We extend Appendix E.1 for deeper discussion about the limitations. Please also refer to the response at **R1Q3.** for the discussion of limitations and what failtures those limitations may result in.
For example, the predicted procedural plan on task "Turking", which refers to "The act or process of performing small tasks using the Amazon Mechanical Turk service." according to Wiktionary. We compare the predicted procedural plan on this task among baselines and our method: (1) The ground truth plan is "Task: Turking. Step 1: Walk to home office.Step 2: Walk to desk.Step 3: Find chair.Step 4: Sit on chair.Step 5: Find computer.Step 6: Switch on computer" (2) The plan predicted by Chain baseline is empty. (3) The plan predicted by LLMaP baseline is "Task: Turking. Step 1: Put teddybear on oven." (4) Our prediction is "Task: Turking. Step 1: Eat food turkey.  Step 2: Drink water.  Step 3: Sleep." We can see that for the "out-of-knowledge" task, our method also lead failure planning. We assume this is mainly due to the limited knowledge in external resources, as discussed in the Appendix E.1, and this main failure mode can be avoided by introducing larger external resources (e.g, Wiktionary), similar as other knowledge-enriched methods. 
We add above analysis in an additional subsection Appendix E.2 to discuss detailed failture modes and examples with analysis in the revision.

> **R2W2RQ2.** Some results, such as Table 1, seem to outperform baselines with larger models. I’m surprised by this as I would think your approach would be particularly important to add structure when LLM’s are more inaccurate. Do you have any intuition on why this might be?

We suppose GPT3 works better given the structured prompt, since they may see similar data. Thus when the correct structure is provided by our model, the larger models (e.g., GPT3 over GPT2) could benefit more and achieve larger performance gain.

### Minor Notes
> **R2M(inor)N(ote)1.**  “The Termination Condition is either reaching the max step t or the matching score is below threshold θ. “ Instead of thresholding, one can compare to an end of statement token’s probability.

We follow the termination condition in Zero-shot Planner (Huang et al.), because the procedural planning is also temporally extended. The end of statement token is also a promising termination condition, we try it for the baselines and our method by appending the final step "End of the task" to all the ground truth procedural plans. However, this termination condition works on the GPT3 base architecture, but not works on the GPT2 and BART. We suppose it's due to that the experiment is conducted under zero-shot setting by prompting the large language models, and thus the end of statement condition is not universally ideal for the large language models.

> **R2MN2.**  Mention in the intro where the common sense external knowledge comes from (though I know it is in Figure 1).

We clarify the external knowledge resources (e.g., ConceptNet) in the introduction of the revision.

> **R2MN3.** How do you extract entity names from the task name?

As mentioned in Section 3.1 (Stage 1): "As for the implementation,  the high-level task name $T$ is Semantically Parsed into the Entity Set $T_E$ with the named entity information in order to extract the representative nodes from the graph. We use NLTK to tokenize and \texttt{pos\_tag} the task text. Then we use the noun (e.g. television), noun phrases (e.g. remote control), and verb phrases (e.g. watch television) as the entity node."
We re-write the paragraph to highlight the implementation of how we extract entity names from the task name in the revision.

> **R2MN4.** “show that pre-trained knowledge (D) in LLMs confounds” What is D here?

The pre-trained knowledge ($D$) is biased to some correlation existed in the pre-training data, and thus is a confounder. For example, as shown in Figure 2, living room and TV is highly correlated in human-annotated training dataset, $D$ in LLMs is a biased prior that assume $P(TV|*living room*) \rightarrow 1$. However it's not always the case that the next plan of go to living room is watch TV, or that when the task is watch TV, you need to go to living room.

> **R2MN5.** “We describe the implementation of such frontdoor adjustment in Section 3.1.” but section 3.1 is 2 pages long, be more specific.

To achieve our front-door adjustment, we inject external knowledge into LLMs with a neuro-symbolic approach by $3$ stages: 1) Intervention on $T$ and $S_{i-1}$ (Stage1 in Section3.1) 2) Intervention on $P_{i-1}$ (Stage2 in Section 3.1) 3) Full temporal-extended intervention on the aggregation of 1) and 2) (Stage3 in Section 3.1).
We add above specific description in Section 2.2 in the revision.

> **R2MN6.**  Table 3 bolds 0.433 in the button right, though GPT3 + Chain outperforms it with 0.471

We check the result files again, and this is the full metric output for GPT3 + Chain on WikiHow in Table $3$: {"sentence-bleu": 0.09465079848425888, "wmd": 0.9433102857150133, "bert-score-f": 0.8395531213283539, "rouge-1-f": 0.3936172366157493}. We're sorry that the ROUGE-f1 on WikiHow was occassionally pasted from the nubmers on RobotHow. We've used a script file to automatically check the table nubmers in latex format with the raw text output files to ensure the correctness of all other table numbers. And we fixed the number $0.471$ (this is the ROUGE-f1 on RobotHow) as the correct one $0.393$ (this is the actual ROUGE-f1 on WikiHow) in Table 3 in the revision.

> **R2MN7.** “PLAN surpasses powerful baselines (Chain of Thoughts (Wei et al., 2022) and Zero-shot Planner (Huang et al.)) by large margins on both the original and the counterfactual samples.” Are these baselines powerful? They don’t have external information except their prompts.

The Chain of Thoughts (Wei, et al., 2022 baseline utilize additional annotation of Chain of Thoughts exemplar for each task domain. The Zero-shot Planner (Huang, et al.) baseline utilize additional held-out exemplars for each task domain. And then these two baselines will retrieve the most relevant exemplar to the current task, and use it as the prompt. Thus, these baselines are powerful in a way that they directly use human-written procedural plan exemplar, which already contains procedural knowledge in the task-domain.
However, we devise a technique that follow the inspiration from our causal analysis of procedural planning to automatically structuralize such knowledge from the external resources and inject into LLMs.
Surprisingly, our method that do not specify task domain (either WikiHow or RobotHow) still surpass these baselines that leverage the knowledge from the task domain itself.

## Response to Official Review of Paper822 by Reviewer ai1E
### Weaknesses
> **R3W(eakness)1.** Discussion on the failure cases is currently missing. In addition, the generated procedural plan of the proposed method was shown, but it would be interesting and useful for readers to see the exact intermediate outputs of the proposed framework given an actual task from the evaluation dataset, e.g.,  Gs,  PG,  P^G, etc. In this way, readers may have a better understanding of the current capabilities of each module of the proposed framework.

1. **Failure Cases**
We extend Appendix E.1 for deeper discussion about the limitations and add a new Appendix E.2 for filure cases discussion. Please also refer to the response at **R1Q3.** and **R2W2RQ1** for the details, where we analyze the failure case of the task "Turking". The word "Turking" refers to "The act or process of performing small tasks using the Amazon Mechanical Turk service." according to Wiktionary.
We recall the example shown in **R2W2RQ1.** and Appendix E.2 below:
We compare the predicted procedural plan on this task among baselines and our method: (1) The ground truth plan is "Task: Turking. Step 1: Walk to home office.Step 2: Walk to desk.Step 3: Find chair.Step 4: Sit on chair.Step 5: Find computer.Step 6: Switch on computer" (2) The plan predicted by Chain baseline is empty. (3) The plan predicted by LLMaP baseline is "Task: Turking. Step 1: Put teddybear on oven." (4) Our prediction is "Task: Turking. Step 1: Eat food turkey.  Step 2: Drink water.  Step 3: Sleep." We can see that for the "out-of-knowledge" task, our method also lead failure planning.
3.  As suggested, We show exact intermediate outputs of the proposed framework given an actual task from the evaluation dataset in Appendix D.2.
    
### Some minor issues
> **R3M(inor)I(ssues)1.** “Note that in the path T →D→Si ←Pi, Si is a collider…” (second line of the “Stage1” paragraph), should it be “T←D”? 

Yes, it's a typo. It should be "T←D". We fix it as "T←D→Si ←Pi" in the revision.

> **R3MI2.** It would be good to refer readers to the appendix for definitions of backdoor path, frontdoor adjustment, etc. 

We thank the reviewer for this suggestion. We add more references for readers to the term definitions whenever it's needed in the revision. For example, we point readers to the Appendix as "Please refer to Appendix A.1 for causal preliminaries, Appendix A.2 for the back-door adjustment definition, and Appendix A.3 for the front-door adjustment definition." in the introduction section.

> **R3MI3.** How is the Symbolic Rule Set  R  obtained? 

The Symbolic Rule Set $R$ is obtained by mapping the description of the relations (e.g., $AtLocation$ represent `A is a typical location for B, or A is the inherent location of B. Some instances of this would be considered meronyms in WordNet.') in external knowledge graph (e.g., ConceptNet) to symbolic operations (e.g., $Op\_AtLocation$). We add above details in Stage 2 paragraph in Section 3.1 in the revision.

> **R3MI4.** One more ablation experiment: what if removing the first Translation  LMT  and replacing  P^G  with  PG? 

As suggested, to verify the contribution of the first translation language model $LM_T$ that translate the knowledge prompt $P_G$ into admissible one $\hat{P_G}$, we conduct an additional ablation experiment by simply remove the first $LM_T$ and replace $\hat{P_G}$ with $P_G$ to prompt the LLM for procedural planning. We provide results with comparison with other ablations in Table 13 in Appendix C.2.

> **R3MI5.** Suggesting one relevant work:  [https://arxiv.org/abs/2205.11916](https://arxiv.org/abs/2205.11916)  (manual exemplars not required).

This work shows promsing results on leveraging enormous zero-shot knowledge inside LLMs but seems only work on GPT3 architecture. Besides the generated plans are not structured in a desired format.
We consider it as an interesting relevant work and cite this work in the **Prompt for Large Language Model** paragraph in Section 5 Related Works.

### Clarity, Quality, Novelty And Reproducibility
For clarity, we've updated the draft thoroughly and addressing the comments point-by-point. For reproducibility, we will provide the detailed configuration files and executation script to help reproduce the results.


## Response to Official Review of Paper822 by Reviewer i21n
### Weakness
> **R4W(eakness)1.** the proposed method is may not be entirely novel. people have been adding symbolic reasoning to neural models for awhile, and the finding has always been : "If we can successfully 'hack' the underlying DSL that represented the set of tasks, adding symbolic reasoning would perform well". For instance, these works tend to follow the steps of: 1) identify a set of tasks that would be easily represented with symbolic execution, and 2) devote significant engineering efforts to construct the DSL and a symbolic interpreter to help the neural/llm model make better inferences/plans. 
> this work would be of significant contribution if it can show that steps 1) and 2) can be avoided by using a generic external knowledge base (as shown in figure 3). however the writing is too confusing I cannot be sure if that is the case or not.

1. The novelty and also the main point of our work is to conduct the first thorough causal analysis that show the spurious correlations among goals and steps in the procedural planning task. And previous methods that simply prompt the LLMs with the ememplars are not aware of the cause-effet relations in procedure. After defining the problem and SCM of procedural planning in Section 2, we propose a neuro-symbolic approach to implement the interventions toward the SCM to elicit the unbiased procedural knowledge from LLMs. 
2. The symbolic module is utilized to preserve the structure that is benefitial for procedural planning. We're not manully providing any ground truth symbolic procedures to directly represent the task. And we're automatically generating the commonsense-infused prompts to replace with exemplars that really require manual efforts in the baselines.
3. We do not specify the domain of the tasks or knowledge bases. We're using a generic commonsense knowledge base, that do not direclty relate to the tasks in RobotHow or WikiHow but shared the spirit that these knowledge are required in human daily activities.


### Clarity, Quality, Novelty And Reproducibility
We're still working on improving the writing.
We have made some major revisions to address the calrity and improve part of the writing as suggested. We also ask people from different background to give comments and let us revise more on the writing to make it easy-to-understand.

## Response to Official Review of Paper822 by Reviewer UGe5
### Weakness
> **R5W(eakness)1.**  Probably, the proposed model is not technically sound. In fact, many of the components are not well-defined, and the system looks too complicated. The overall model is not ablated well and is full of tricks.

 1. We re-write the Section 2 and 3 to make it more clear how each component function and contribute to the system.
 2. We're showing the system at a fine-grained level, so that we could show the implementation details guided by the analysis of SCM. This fine-grained depiction of our system make it seems very complex, however this is comparable with other baselines. For example, the method in Zero-shot planner (Huang et al.) can be separted as $4$ stages: (1) retrieve the task-relevant program from held-out exemplars (2) Aggregate the prompt with previous steps as temporally-extended prompt for predicting next step (3) Semantic Generation (similar as Stage $4$ in our paper) (4) Admissible Step Translation (the same as Stage $5$ in our paper). The first two stages can be merged into one, however we separete it into two stages to more clearly explain their connection with the causal analysis in Section 2. Thus we claim that we did not introduce a lot complexity into the sysmte. 
 3. As illustrated above, the complexity of our method and the baselines are comparable. Notice that the baslines addtionally need to extract the program-related exemplars. What we do is to replace that part by constructing  knowledge-aware prompt from the external resources instead of retrieving the expensive exemplars required by the baselines.  And how we extract it is guided by the analysis of Structural Causal Model.
 4. We also empircally show that the computing cost of the baselines and our method is comparable in Table 8 and Table 9.

> **R5W2.**  The proposed model seems to borrow a lot of big concepts, such as neural-symbolic or casual models. However, the specific technical contributions are not very clear, and many problems remain unaddressed. In general, the system looks too complicated. This is not a good paper. A good paper should stick to one major point and show the advantage of this point over previous baselines.

1. We're showing the system at a fine-grained level, so that we could show the implementation details guided by the analysis of SCM. This fine-grained depiction of our system make it seems very complex, however this is comparable with other baselines. For example, the method in Zero-shot planner (Huang et al.) can be separted as $4$ stages: (1) retrieve the task-relevant program from held-out exemplars (2) Aggregate the prompt with previous steps as temporally-extended prompt for predicting next step (3) Semantic Generation (similar as Stage $4$ in our paper) (4) Admissible Step Translation (the same as Stage $5$ in our paper). The first two stages can be merged into one, however we separete it into two stages to more clearly explain their connection with the causal analysis in Section 2. Thus we claim that we did not introduce a lot complexity into the system. Please also refer to the response at  **R5W(eakness)1.**.
2. The computing cost is ignorable as empirically shown in Table 8 and Table 9, which show the computing complexity of our method and the baselines are comparable.
3. The major point of our paper is to enable the system with the ability to be aware of the cause-effect relations in procedures. We describe the causal analysis in Section 2 and explain why external knowledge matters in procedural planning. Then we come to how to implement with the guidance of the causal analysis in Section 3. We leverage neuro-symbolic techniques to implement the intervention operations in the SCM. In general, Section 3 is our approach guided by the analysis in Section 2.
4. As illustrated in above three points, we claim that the complexity of our system is comparable as the baselines. At the same time we achieve significant improvement even without additional exemplars.


> **R5W3.**  Human evaluations are not very objective and cannot be easily reproduced. I fail to see a clear motivation for using expensive human evaluations. Instead, showing a lot of generated procedures is far more beneficial than showing a lot of numbers.

1. Motivation for using human evalutions: Our motivation of using human evaluations share the same spirit with the motivation in the baseline Zero-shot Planner (LLMaP) paper (Huang, et al.): "Unlike most embodied environments where the completion of a task can be easily judged, the ambiguous and multimodal nature of natural language task specification makes it impractical to obtain a gold-standard measurement of correctness. Therefore, we conduct human evaluations for the main methods. ". 
We add a new paragraph that explain the motivation why we use human evaluations in the revision in Appendix C.2: "Since the nature of the procedural planning task can be open-domain in that the golden plans may not be unique. This leads to the challenge that common automatic metrics proposed in natural language task are not perfect to evaluate procedural planning. We assume that the human evaluation on *Coverage* and *Order* can reflect how well the procedural plans are close to human-annotated program, because the human annotators are required to determine whether the task can be completed in any reasonable scenario using the procedural plans explicitly. Thus we provide both the automatic evaluation and human evaluation on two aspects  with description in the Metrics paragraph in Section 4.1."
3. Generated procedures: In addition to showcases in Table 3, we provide a lot of generated procedures of baselines and our method based on two LLMs architectures on two datasets under standard and counterfactual setting in Table 10-14. We also extend Table 10 and Table 11 with more examples to help readers compare the qualitative results.

### Specific Comments
> **R5C(omment)1.**  In the task definition, what are the actions, and what are the object sets? I think in real natural language, the set of actions (described in natural language) or objects can be extremely large. How can the formulation handle this? I did not see the specific usage of these variables. Probably the problem is over-formulated.

Yes, the actions and objects set are extremely large and we do not specify that explicitly. Indeed, the system is aware of the admissible plans set $\bar{S}$ for each task domain. We modify the problem definition as "There exists certain admissible plans $\bar{S}$, which is a fixed set constrained by the task domain $M_T$ (e.g., the affordance of the interacted objects)." And we updated the description in Stage 5 paragraph in Section 3.2 to remove the over-formulated $A$ and $O$ for more accurate definition.


> **R5C2.**  The authors use the same variable D for task D_T and confounding variable D. This is hard to decode.

We change the notation for the task domain from $D_T$ to $M_T$, to seperate from the variable $D$ for better clarity.

> **R5C3.** This paper is related to program-guided works [1-2]. A deep discussion is recommended.

These two program-guided works aim to utlize human written programs in a formal language as a precise and expressive way to specify task, and thus avoid ambiguity of natural language instructions. Our method is guided by the intuition of our thorough causal analysis of the procedural planning task and come to the solution of constructing prompt from external resources in a neuro-symbolic approach.
We add the discussion about these two program-guided workds in related work (Procedural Planning in Section 5) in the revision.

> **R5C4.**  I can hardly understand the implementation of the SCM. What are the input and output of the SCM? Is there any replacement (e.g. standard transformers) for this module? What is the sample output of the SCM? Is there any reference to the SCM? Take Figure 2 as an example; how does the SCM forward the reasoning path? How does the SCM encode the action and object? How does the SCM produce the output? These problems are still unclear to me.

We follow the definition of Structural Causal Model (SCM) in causal inference literatures ([1,2]). The earliest version of SCM is introduced in [3]. The SCM is commonly represented with causal graphs (entension of directed acyclic graphs) that express the causal relationships between variables in a system ([4,5]). We include the causal prelimiaries in Appendix A.1.
For better clarity, we refer readers to these definitions in the introduction section as "Please refer to Appendix A.1 for causal preliminaries, Appendix A.2 for the back-door adjustment definition, and Appendix A.3 for the front-door adjustment definition." in the revision main paper.
Basically we first define the SCM in Figure 2 to describe the causal relationship among variables in the procedural planning task. The SCM is actually a causal graph modeling with abstract nodes and edges, instead of something like a neural network "model" (e.g., transformer) that take some input and produce the output. After defining our SCM, we propose to apply front-door adjustment to solve the spurious correlation (Figure 2(b)). To achieve the front-door adjustment, we devise an architecture (Figure 3) which can be separated in $5$ stages (Section 3.1 and 3.2).

[1] Noah Weber, Rachel Rudinger, and Benjamin Van Durme. 2020. [Causal Inference of Script Knowledge](https://aclanthology.org/2020.emnlp-main.612). EMNLP, pages 7583–7596, Online. Association for Computational Linguistics.
[2] X. Yang, H. Zhang and J. Cai, "Deconfounded Image Captioning: A Causal Retrospect," in _IEEE Transactions on Pattern Analysis and Machine Intelligence_, doi: 10.1109/TPAMI.2021.3121705.
[3] [Wright, S. (1921). “Correlation and causation”. Journal of Agricultural Research. 20: 557–585.](https://naldc.nal.usda.gov/download/IND43966364/pdf)
[4] [Structural Causal Models](https://www.causalflows.com/structural-causal-models/)
[5] [Edward N. Zalta, 2018, "Causal Models", The Stanford Encyclopedia of Philosophy](https://plato.stanford.edu/entries/causal-models/)


> **R5C5.** Why does procedural planning need so many steps (five-stage pipelines)? I see that motivation is to fuse different motivations (task definition, previous steps, and external knowledge). If so, why not encode this information in parallel so that the fused (e.g. concatenation) information can be used in downstream tasks?

Please refer to the response at **R5W(eakness)1.** and **R5W2.**, where we explain why the complexity of the baselines and our approach are comparable. Basically, our implementation at Section 3 is guided by the causal analysis in Section 2. We separate the sysmte into a more fine-grained level ($5$ stages) to make it easier to connect with the intuition from Section 2, Figure 2 and Figure 4. Each stage either refer to the operation in the SCM or the generation process. We're fusing the  information togerther, but the motivation is more into how we inject the external knowledge to mitigate the biased pre-trained knowledge $D$. 

> **R5C6.**  Algorithm 1 is a waste of space, and it is better to replace it with a figure (or make figure 3 better).

We're working on making Figure 3 better to replace with Algorithm 1, and perhaps move Algorithm 1 to Appendix to save space. We added an additional zoomed in algorithm block for Section 3.1 in Algorithm 1.

> **R5C7.**  Many concrete designs, such as the symbolic executors, are missing. It seems that the symbolic executors are trivial and can be easily learned. In other words, I do not think the "neural-symbolic" stuff in the title plays an important role in this system. In fact, what is neural symbolic in this line of work? Why is it important? How to connect the big concept with the experimental results with the LLMs? These questions are far more important to show than the ad-hoc model designs.

We first show our causal analysis in Section 2 and then we show how we implement the operations in SCM in Section 3. Specifically, we leverage a neuro-symbolic approach to construct commonsense-infused prompts, which preserve the structural knowledge. We show the ablation without symbolic module in Table 3, which experience the performance drop in the LLMs.

### Clarity, Quality, Novelty And Reproducibility
> - "The major limitation is the clarity and the paper presentation." "However, if I do not see a major revision in the rebuttal phase in the writing parts clarifying the related concerns, I might decide to reject this paper."

We thank the reviewer for recognizing the good directions and good ideas of our work. And we make a thorough revision that address each reviewer's concerns point-wisely for clarity. In addtion, we made a major revision of the writing and absorb writing improving opinions of researchers from different background to make sure our paper is more clear and easy-to-follow.

## SmartyPants

SmartyPants converts ASCII punctuation characters into "smart" typographic punctuation HTML entities. For example:

|                |ASCII                          |HTML                         |
|----------------|-------------------------------|-----------------------------|
|Single backticks|`'Isn't this fun?'`            |'Isn't this fun?'            |
|Quotes          |`"Isn't this fun?"`            |"Isn't this fun?"            |
|Dashes          |`-- is en-dash, --- is em-dash`|-- is en-dash, --- is em-dash|


## KaTeX

You can render LaTeX mathematical expressions using [KaTeX](https://khan.github.io/KaTeX/):

The *Gamma function* satisfying $\Gamma(n) = (n-1)!\quad\forall n\in\mathbb N$ is via the Euler integral

$$
\Gamma(z) = \int_0^\infty t^{z-1}e^{-t}dt\,.
$$

> You can find more information about **LaTeX** mathematical expressions [here](http://meta.math.stackexchange.com/questions/5020/mathjax-basic-tutorial-and-quick-reference).


We thank the reviewer for bringing out above concerns and that we could explicitly explain it and add these interesting discussions in the paper revision.

~~e.g. , when our causal analysis break(tricky to bring out this issue)~~
~~better to discuss when the implementation break 
@ also ask xinyi ~~
It's possible in some extreme situation, the commonsense-infused prompt is not ta, and thus the constructed $P_i$ do not hold the front-door criterion. map to which step is an issue in SCM => if the multi-hop is an limitation, then which part of causal analysis is a problem.

We're sorry that the numbers for GPT3 + Chain on WikiHow (four metrics including ROUGE-f1: 0.471) were first pasted from its performance numbers on RobotHow (four metrics including ROUGE-f1:0.471) just to expand the table format on the right part. And then they're manually replaced by the output results on WikiHow. And

**consider add a small experiment or some examples comparison for end of statement condition** 
"Task: how to make coffee Step 1: go to kitchen Step 2: switch on the coffee machine Step 3: pour coffee in the cup Step 4: grab the cup Step 5: switch off the coffee machine Step 6: End of the Task  Task: how to make breakfeast Step 1: go to kitchen Step 2: get the food that you want Step 3: put the food in the oven Step 4: wait until the food is ready Step 5: take the food out of the oven Step 6: put the food on the table Step 7: End of the Task"

and modify Figure 3 with stage information


% rebuttal reference https://arxiv.org/pdf/2003.03923.pdf
